List Decodable Subspace Recovery

Learning from data in the presence of outliers is a fundamental problem in statistics. In this work, we study robust statistics in the presence of overwhelming outliers for the fundamental problem of subspace recovery. Given a dataset where an $\alpha$ fraction (less than half) of the data is distributed uniformly in an unknown $k$ dimensional subspace in $d$ dimensions, and with no additional assumptions on the remaining data, the goal is to recover a succinct list of $O(\frac{1}{\alpha})$ subspaces one of which is nontrivially correlated with the planted subspace. We provide the first polynomial time algorithm for the 'list decodable subspace recovery' problem, and subsume it under a more general framework of list decoding over distributions that are "certifiably resilient" capturing state of the art results for list decodable mean estimation and regression.

==> antiConcentration.tex <==
\section{Certifying Anticoncentration}\label{sec:anticoncentration}
%

Anticoncentration is a measure of the "spread" of a distribution.  For any distribution $\cD$, let $\eta$ be a parameter $0 < \eta < \frac{1}{2}$.  If the probability mass of $\cD$ contained in the $\eta$ interval around the origin is small, than $\cD$ is anticoncentrated.  For example, in the case of $\cD = \cN(0,1)$, the mass of $\cD$ in any $\eta$ interval about the origin is upper bounded by $\frac{2}{\sqrt{2\pi}}\eta$.  This property of the probability mass decaying linearly with $\eta$ as $\eta$ goes to zero is what motivates the following definition.   



\begin{definition}\label{def:anticoncentration}
    A probability distribution $\cD$ over $\R^d$ is said to be $c$-anticoncentrated if for any $0 < \eta < \frac{1}{2}$ there exists $\tau \leq c\eta$ such that for any measurable subset $\cE \in \R^n$, and for all $v \in \R^d$ with $\norm{v} \leq 1$, we have that
    $$ \E[ \iprod{X,v}^2 \cdot \Ind[\cE] ] \geq \eta^2 \cdot \Pr[\cE]  \cdot \norm{v}^2 - \eta^2\tau$$ 
\end{definition}
\Pnote{$\Omega$ is undefined here. We should probably define $\cE$ to be a measurable subset of $\R^n$}


We now state the SoS version of anticoncentration
\begin{definition}\label{def:anticoncentration}
Let $D: [0,1/2] \to \N$.
%
A probability distribution $\cD$ over $\R^d$ is said to $(c, D(\eta))$-SoS-anticoncentrated, 
%
If for any $0 < \eta < \frac{1}{2}$ there exists $\tau \leq c\eta$ and there exists a constant $k \in \N$ such that for all $N > d^k$,
with probability $1-d^{-k}$, over samples $x_1,\ldots, x_N \sim \cD$ the following polynomial system

$$
\cP = \left\{
        \begin{array}{ll}
            w_i^2 = w_i & i \in [N]\\
    \norm{v}^2 \leq \rho^2 \\
    \norm{\frac{1}{N}\sum_{i=1}^N X_i^{\otimes \frac{t}{2}}(X_i^{\otimes \frac{t}{2}})^T - M_t} < \epsilon& t \in [k]\\
        \end{array}
    \right.
$$
yields a degree $D(\eta)$ SoS proof of the following inequality 

\begin{align*}
    \cP\SoSp{D(\eta)}\Big\{\frac{1}{N}\sum_{i = 1}^N w_i \iprod{X_i,v}^2 \geq \eta^2 (\frac{1}{N}\sum_i w_i) \norm{v}^2 - \eta^2 \tau \rho^2\Big\}
\end{align*}
\end{definition}

\Pnote{good to remind the reader what $M_t$ denotes in the above definition.  Perhaps, we should uniformly use $M_4(\cD)$?}

\begin{theorem}\label{thm:anti-sufficient} (Sufficient conditions for SoS anti-concentration)
If the degree $D(\eta)$ empirical moments of $\cD$ converge to the corresponding true moments $M_t$ of $\cD$, that is for all $t \leq D(\eta)$ 
$$
\lim_{N \rightarrow \infty}\Norm{\frac{1}{N}\sum_{i=1}^N X_i^{\otimes \frac{t}{2}}(X_i^{\otimes \frac{t}{2}})^T - M_t} = 0 
$$
And if there exists a uni-variate polynomial $I_{\eta}(z) \in \R[z]$ of degree at most $D(\eta)$ such that 
\begin{enumerate}
    \item $I_{\eta}(z) \geq 1-\frac{z^2}{\eta^2\rho^2}$ for all $z \in \R$.
    \item $\cP\SoSp{D(\eta)} \Big\{\norm{v}^2 \cdot \E_{x \in \cD}[I_{\eta}(\iprod{v, x})] \leq c\eta\rho^2\Big\}$.
\end{enumerate}
Then $\cD$ is $(c,D(\eta))$ certifiably anticoncentrated.

\end{theorem}

\begin{lemma}\torestate{\label{lem:normal-anti}
For every $d \in \N$, the standard Gaussian distribution $\cN(0,I_d)$ is $(c,O(\frac{1}{\eta^4}))$-SoS-anticoncentrated. In particular there exists a construction for $c \leq 2\sqrt{e}$}    
\end{lemma}

\begin{comment}
\begin{theorem} There exists a degree $T$ sum of squares proof of the following polynomial inequality for $0 < ||v|| < \rho$
\begin{align*}
    \frac{\delta\rho}{\sqrt{2\pi}}+ \frac{\rho^2}{\delta^2}\frac{1}{\beta N}\sum\limits_{i=1}^N w_iw_i'\langle X,v\rangle^2 \geq  \frac{1}{\beta N} \sum\limits_{i=1}^N w_iw_i'||v||^2
\end{align*}
\end{theorem}
\end{comment}
First we will prove \pref{thm:anti-sufficient}

\begin{proof} (\pref{thm:anti-sufficient})
First, it is a standard fact that every uni-variate polynomial inequality has a sum of squares proof.  More precisely, for any $p(x) \in \R[x]$ satisfying $p(x) \geq 0$, then it is true that $p(x) \SoSge_{\text{deg}(p(x))} 0$.  Furthermore, this is also true over any interval $[a,b] $

\begin{fact}\label{fact:univar}
Let $a < b$. Then, a degree $2d$ polynomial $p(x)$ is non-negative on $[a, b]$, if and only if it can be written as
$$
\left\{
\begin{array}{ll}
     & p(x) = s(x) + (x - a)(b - x)t(x), \text{    if deg(p) is even}\\
    & p(x) = (x - a)s(x) + (b - x)t(x), \text{     if deg(p) is odd}\\
\end{array}
\right.
$$
where $s(x)$, $t(x)$ are SoS. In the first case, we have $deg(p) = 2d$, and $deg(s) \leq 2d$, $deg(t) \leq 2d - 2$. In
the second, $deg(p) = 2d + 1$, and $deg(s) \leq 2d$, $deg(t) \leq 2d$.
\end{fact}
In light of this fact, we use \pref{thm:anti-sufficient} condition 1 to lower bound $\iprod{X_i,v}^2$ by 

\begin{align*}
\cP \SoSp{D(\eta)} \langle X,v\rangle^2 \geq \eta^2\rho^2(1 - I_\eta(\langle X_i,v\rangle))
\end{align*}
Therefore, 
\begin{align*}
    \cP \SoSp{D(\eta)}\sumn w_iw_i'\langle X,v\rangle^2 \geq \sumn w_iw_i'\eta^2\rho^2 (1 - I_{\delta}(\langle X_i,v\rangle))
\end{align*}
Then using the certificate that $\{\norm{v}^2 < \rho^2\}$ we obtain
\begin{align*}
    \cP \SoSp{D(\eta)}\sumn w_iw_i'\eta^2\rho^2(1 - I_{\eta}(\langle X_i,v\rangle)) \geq \sumn w_iw_i'\eta^2\norm{v}^2 (1 - I_{\eta}(\langle X_i,v\rangle))
\end{align*}

\begin{align*}
    = \sumn w_iw_i'\eta^2\norm{v}^2 - \sumn w_iw_i'\eta^2\norm{v}^2I_{\eta}(\langle X_i,v\rangle)
\end{align*}
Then using the fact that $I_\eta(\langle X_i,v\rangle)$ is SoS and $\{w_i^2 = w_i\} \SoSp{} (1 - w_i) \SoSge_2 0$, we subtract $\sumn w_i'(1-w_i)I_\eta(\langle X_i,v\rangle)$ to obtain 

\begin{align*}
    \geq \sumn w_iw_i'\eta^2\norm{v}^2 - \eta^2 \norm{v}^2\sumn w_i'I_{\eta}(\langle X_i,v\rangle)
\end{align*}

Expanding out $I_\delta(\langle X_i,v\rangle)$ as a degree $D(\eta)$ polynomial with coefficients $\alpha_1,...,\alpha_{D(\eta)}$ we have

\begin{align*}
    I_\eta(\langle X_i,v\rangle) = \sum_{t=1}^T \alpha_t \langle X_i,v\rangle^t
\end{align*}
We want replace the empirical average $\sumn w_i' I_\eta(\langle X_i,v\rangle)$ with the expectation $\E_{X \sim N(0,I)} I_\eta(\langle X,v \rangle)$ and bound the error term.  Indeed, we know that
\begin{align*}
     \sumn w_i'I_\eta(\langle X_i,v\rangle) = \sum\limits_{t=1}^T \alpha_t\sumn w_i'\langle X_i,v\rangle^t  = \sum\limits_{t=1}^{D(\eta)} \alpha_t\big \langle \sumn w_i' X_i^{\otimes \frac{t}{2}}(X_i^{\otimes\frac{t}{2}})^T, v^{\otimes \frac{t}{2}}(v^{\otimes\frac{t}{2}})^T \big\rangle
\end{align*}

 
\begin{align*}
    = \sum\limits_{t=1}^T \alpha_t\big \langle \sumn w_i' X_i^{\otimes \frac{t}{2}}(X_i^{\otimes\frac{t}{2}})^T - \E_{X \sim N(0,I)} X^{\otimes \frac{t}{2}}(X^{\otimes\frac{t}{2}})^T, v^{\otimes \frac{t}{2}}(v^{\otimes\frac{t}{2}})^T \big\rangle + \sum\limits_{t=1}^{D(\eta)} \alpha_t\big \langle \E_{X \sim N(0,I)} X^{\otimes \frac{t}{2}}(X^{\otimes\frac{t}{2}})^T, v^{\otimes \frac{t}{2}}(v^{\otimes\frac{t}{2}})^T \big\rangle
\end{align*}

Then by degree $D(\eta)$ SoS Cauchy Schwarz we obtain
\begin{align*}
    \SoSle  \sum\limits_{t=1}^{D(\eta)} \alpha_t\norm{\sumn w_i' X_i^{\otimes \frac{t}{2}}(X_i^{\otimes\frac{t}{2}})^T - M_t}_F^2 \norm{v}^t + \sum\limits_{t=1}^{D(\eta)}\alpha_t\E_{X \sim N(0,I)}\langle X,v\rangle^t
\end{align*}
Thus for our setting of $N$ and $d$ we obtain,
\begin{align}\label{eq:anti1}
 = \E_{X \sim N(0,I)}I_\eta(\iprod{X_i,v}) + o_d(1)
\end{align}
Note that it is important that the coefficients of $I_\eta(z)$ are chosen independently of $d$ or at the very least don't grow too fast with respect to $d$. Our final bound is, 

\begin{align*}
    \cP \SoSp{D(\eta)}\sumn w_iw_i'\langle X,v\rangle^2 \geq \sumn w_iw_i'\eta^2\norm{v}^2 - \eta^2 \norm{v}^2\E_{z \sim N(0,\norm{v}^2)} I_{\eta}(z) + o_d(1)
\end{align*}
Applying sufficient condition 2 we obtain 
\begin{align*}
    \cP\SoSp{D(\eta)}\Big\{\frac{1}{N}\sum_{i = 1}^N w_i \iprod{X_i,v}^2 \geq \eta^2 (\frac{1}{N}\sum_i w_i) \norm{v}^2 - \eta^2 \tau\rho^2 \Big\}
\end{align*}
as desired.  
\begin{comment}
Consider the second term which we need to upper bound.  For $||v|| < \frac{1}{2\pi}^{1/4}\sqrt{\delta\rho}$ we have

\begin{align*}
    \delta^2 \frac{||v||^2}{\rho^2}\E_{z \sim N(0,||v||^2)} I_{\delta}(z) \leq \frac{\delta^3}{\sqrt{2\pi}\rho}
\end{align*}

Where we trivially upper bound the expectation by $1$.
And for $||v|| > \frac{1}{2\pi}^{1/4}\sqrt{\delta\rho}$ we have

\begin{align*}
    \delta^2 \frac{||v||^2}{\rho^2}\E_{z \sim N(0,||v||^2)} I_{\delta}(z) \leq  \delta^2 \frac{||v||^2}{\rho^2}\frac{1}{\sqrt{2\pi}||v||} \delta \leq \frac{\delta^3}{\sqrt{2\pi}\rho}
\end{align*}

Where we upper bounded $||v|| < \rho$.  Thus we have the following lower bound uniformly over $0 < ||v|| < \rho$
\begin{align*}
    \frac{1}{\beta N} \sum\limits_{i=1}^N w_iw_i'\langle X,v\rangle^2 \geq  \frac{1}{\beta N} \sum\limits_{i=1}^N w_iw_i'\delta^2 \frac{||v||^2}{\rho^2} - \frac{\delta^3}{\sqrt{2\pi}\rho}
\end{align*}

Rearranging terms we have,
\begin{align*}
    \frac{\delta^3}{\sqrt{2\pi}\rho}+ \frac{1}{\beta N}\sum\limits_{i=1}^N w_iw_i'\langle X,v\rangle^2 \geq  \frac{1}{\beta N} \sum\limits_{i=1}^N w_iw_i'\delta^2 \frac{||v||^2}{\rho^2}
\end{align*}

Multiplying both sides by $\frac{\rho^2}{\delta^2}$ we conclude

\begin{align*}
    \frac{\delta\rho}{\sqrt{2\pi}}+ \frac{\rho^2}{\delta^2}\frac{1}{\beta N}\sum\limits_{i=1}^N w_iw_i'\langle X,v\rangle^2 \geq  \frac{1}{\beta N} \sum\limits_{i=1}^N w_iw_i'||v||^2
\end{align*}

Eventually we will have

\begin{align*}
   \frac{1}{\beta N} \sum\limits_{i=1}^N w_iw_i'||v||^2 \leq \frac{\delta\rho}{\sqrt{2\pi}}+ \frac{4\rho^2\sigma^2}{\delta^2}
\end{align*}

Setting $\delta = \frac{\beta \rho}{4}$ we obtain

\begin{align*}
   \frac{1}{\beta N} \sum\limits_{i=1}^N w_iw_i'||v||^2 \leq \frac{\beta\rho^2}{4\sqrt{2\pi}}+ \frac{\sigma^2}{\beta^2}
\end{align*}

Matching this with global correlation of $\frac{\rho^2\beta}{4}$ we contract the problem from $\rho$ to $\frac{\rho}{2}$
\end{comment}
\end{proof}





==> main.tex <==



\section{Introduction }
Problem Setup:  Given data $X_1,X_2,..,X_N \in \mathbb{R}^d$.  A fraction $\beta \in [0,1]$ of the points are drawn i.i.d from a $(k,l)$-certifiably subgaussian distribution.  The remaining $(1-\beta)N$ points can be adversarially chosen.










==> prelims.tex <==
\section{Preliminaries}
\label{sec:prelims}
Here we present the basic definitions and properties of sum of squares proofs, and their relationship with pseudodistributions and pseudoexpectations. For a more detailed treatment see \cite{DBLP:conf/stoc/BarakBHKSZ12}.  

\subsection{Sum-of-Squares Toolkit} \label{SoS-toolkit}
\paragraph{Sum-of-Squares Proofs}
For any nonnegative polynomial $p(x): \R^d \rightarrow \R$, one could hope to prove its nonnegativity by writing $p(x)$ as a sum of squares of polynomials $p(x) = \sum_{i=1}^m q_i(x)^2$ for a collection of polynomials $\{q_i(x)\}_{i=1}^m$.  Such a proof would be succinct and easy to verify.  Unfortunately, there exist nonnegative polynomials with no sum of squares proof even for $d = 2$.  Nevertheless, there is a generous class of nonnegative polynomials that admit a proof of positivity via a proof in the form of a sum of squares.  The key insight of the sum of squares algorithm, is that these sum of squares proofs of nonnegativity can be found efficiently provided the degree of the proof is not too large.  We begin with a rough overview of sum of squares proofs, their dual object pseudoexpectations, and then present the guarantees of the SoS algorithm.      

\begin{definition} (Sum of Squares Proof)
Let $\mathcal{A}$ be a collection of polynomial inequalities $\{p_i(x) \geq 0\}_{i=1}^m$.  A sum of squares proof that a polynomial $q(x) \geq 0$ for any $x$ satisfying the inequalities in $\mathcal{A}$ takes on the form 

\[
    \left(1+ \sum_{k \in [m']} b_k^2(x)\right) \cdot q(x) = \sum_{j\in [m'']} s_j^2(x) + \sum_{i \in [m]} a_i^2(x) \cdot p_i(x) \mcom
\]
where $\{s_j(x)\}_{j \in [m'']},\{a_i(x)\}_{i \in [m]}, \{b_k(x)\}_{i \in [m']}$ are real polynomials.  If such an expression were true, then $q(x) \geq 0$ for any $x$ satisfying $\mathcal{A}$.  We call these identities sum of squares proofs, and the degree of the proof is the largest degree of the involved polynomials $\max \{\deg(s_j^2), \deg(a_i^2 p_i)\}_{i,j}$.  Naturally, one can capture polynomial equalities in $\mathcal{A}$ with pairs of inequalities.   We denote a degree $\ell$ sum of squares proof of the positivity of $q(x)$ from $\cA$ as $\cA \sststile{\ell}{x} \{q(x) \geq 0\}$ where the superscript over the turnstile denote the formal variable over which the proof is conducted.  This is often unambiguous and we drop the superscript unless otherwise specified.    
\end{definition}

Sum of squares proofs can also be strung together and composed according to the following convenient rules.  

\begin{fact}
For polynomial systems $\cA$ and $\cB$, if $\cA \sststile{d}{x} \{p(x) \geq 0\}$ and $\cB \sststile{d'}{x} \{q(x)\geq 0\}$ then $\cA \cup \cB \sststile{\max(d,d')}{x}\{p(x) + q(x) \geq 0\}$.  Also $\cA \cup \cB \sststile{dd'}{x} \{p(x)q(x) \geq 0\}$ 
\end{fact}
We now turn to pseudoexpectations, the dual object to SoS proofs.  

\paragraph{Pseudoexpectations}
%, we can write an SDP of size $n^{O(d)}$ which finds a degree-$d$ sum-of-squares refutation, if one exists (see \cite{rothvoss2013lasserre} for more discussion).
%
%If there is no degree-$d$ refutation, the dual semidefinite program computes in time $n^{O(d)}$ a linear functional over degree-$d$ polynomials which we term a {\em pseudoexpectation}.

\begin{definition}
a degree $\ell$ pseudoexpectation $\pE : \R[x]_{\leq \ell} \to \R$ {\it satisfying $\cP$} is a linear functional over polynomials of degree at most $\ell$ satisfying $\pE[1] = 1$, $\pE[p(x) a^2(x)] \geq 0$ for all $p \in \cP$ and polynomials $a$ such that $\deg(a^2 \cdot p) \le \ell$, and $\pE[q(x)^2] \ge 0$ whenever $\deg(q^2) \le \ell$.
\end{definition}
Just as expectations are taken over distributions, pseudoexpectations are identified with a pseudodistribution $\zeta$.  Thus we often write $\pE_{\zeta}$ dropping the pseudodistribution notation when the pseudoexpectation we are working with is obvious from context.  

\begin{fact} (Informal Soundness)
The properties of the pseudoexpecation imply that $\cA \sststile{r}{x} \set{q(x) \ge 0}$, then if $\pE$ is a degree-$\ell$ pseudoexpectation operator for the polynomial system defined by $\cA$, then $\pE[q(x)]  \ge 0$.
\end{fact}

%\begin{claim}\label[claim]{cl:SoS-cs}
%    If $\pE$ is a degree-$d$ pseudoexpectation and if $p,q$ are polynomials of degree at most $\frac{d}{2}$, then $\pE[q(x)\cdot p(x)] \le \frac{1}{2}\pE[q(x)^2] + \frac{1}{2}\pE[p(x)^2]$.
%\end{claim}


\paragraph{SoS Algorithm}
The degree $D$ moment tensor of a pseudoexpectation $\pE_{\zeta}$ is the tensor $\pE_\zeta(1, x_1, x_2, . . . , x_n)^{\otimes D}$.
Each entry corresponds to the pseudo-expectation of all monomials of degree at most $D$ in x. The set of all degree-$D$ moment tensors of degree $D$ pseudoexpectations is convex, and there's a separation oracle that runs in time $n^{O(D)}$.

\begin{fact} (\cite{Nesterov00}, \cite{Parrilo00}, \cite{Lasserre01}, \cite{Shor87}). For any $n$, $D \in \Z^+$, let $\pE_{\zeta}$ be degree $D$ pseudoexpectation satisfying a polynomial system $\cP$.  Then the following set has a $n^{O(D)}$-time weak
separation oracle (in the sense of \cite{GLS1981}):
 \begin{align*}
 & \{\pE_\zeta(1, x_1, x_2, . . . , x_n)^{\otimes D}| \text{ degree } D \text{ pseudoexpectations } \pE_{\zeta} \text{ satisfying }\cP \}
\end{align*}

Armed with a separation oracle, the ellipsoid algorithm finds a degree $D$ pseudoexpectation in time $n^{O(D)}$, which we call the degree $D$ sum-of-squares algorithm. 
\end{fact}

Next we present some useful inequalities captured by the sum of squares proof system

\paragraph{Useful Inequalities}

\begin{fact} (Cauchy Schwarz)
Let $x_1,..,x_n,y_1,...,y_n$ be indeterminates, than 

$$\sststile{4}{} \big(\sum_{i \leq n}x_iy_i\big)^2 \leq \big(\sum_{i \leq n}x_i^2\big)\big(\sum_{i \leq n}y_i^2\big) $$
\end{fact}

\begin{fact} (Triangle Inequality) 
Let $x,y$ be $n$-length vectors of indeterminates, then 
$$\sststile{2}{} \norm{x + y}^2 \leq 2\norm{x}^2 + 2\norm{y}^2 $$
\end{fact}


\begin{fact}\label{fact:pseudocauchy}(Pseudoexpectation Cauchy Schwarz). 
Let $f(x)$ and $g(x)$ be degree at most $\ell \leq \frac{D}{2}$ polynomial in indeterminate $x$, then $$\pE[f(x)g(x)]^2 \leq \pE[f(x)^2]\pE[g(x)^2]$$  
\end{fact}

\begin{fact} (Spectral Bounds)
Let $A \in \R^{d \times d}$ be a positive semidefinite matrix with $\lambda_{max}$ and $\lambda_{min}$ being the  largest and smallest eigenvalues of $A$ respectively. Let $\pE$ be a pseudoexpectation with degree greater than or equal to $2$ over indeterminates $v = (v_1,...,v_d)$.  Then we have 
$$\sststile{2}{} \iprod{A,vv^T} \leq \lambda_{max} \norm{v}^2 $$
and 
$$\sststile{2}{} \iprod{A,vv^T} \geq \lambda_{min} \norm{v}^2 $$
\end{fact}

\begin{remark}
(Numerical accuracy). To make our error guarantees precise, we have to discuss issues of bit complexity.  
The SoS algorithm obtains a degree $D$ pseudoexpectation $\pE_\zeta$ satisfying polynomial system $\cP$ approximately.  That is to say, for every $g$ a sum of squares and $p_1, . . . , p_\ell \in \cP$
with deg$[g \prod p_i \leq D]$, one has $\pE g\prod_{i \in \cP} p_i \geq - 2^{-\Omega(n)} \norm{g}$, where $\norm{g}$ is $\ell_2$ norm of the coefficients
of $g$.  So long as all of the polynomials involved in our SoS proofs have coefficients bounded by $n^B$ for some large constant $B$, then for any polynomial system $\cQ$ such that $\cP \sststile{}{} \cQ$, we have $\cQ$ satisfied up to error $2^{-\Omega(n)}$.
\end{remark}
      





==> regressionoverview.tex <==

\section{Technique Overview: Robust Regression}\label{sec:reg-overview}
In this section we introduce many of the ideas involved in designing our rounding algorithm. We leave sharper error/runtime guarantees and general distributional assumptions to later sections.


Let $N$ be the size of the data set.  Let $\beta < \frac{1}{2}$, and let $M = \beta N$.    
We receive a data set $\cD = \{(X_i,y_i)\}_{i=1}^N$ where the $X_i \in \R^d$ are the covariates and the $y_i \in \R$ are the labels.  Of the covariates, $M$ points are drawn $X_i \sim \cN(0,I)$.  We will refer to these points as "inliers".  Furthermore, we introduce boolean variables $w_1',...,w_N' \in \{0,1\}$ indicating if a data point is an inlier, equal to $1$; outlier, equal to $0$.  Let $\ell' \in \R^d$ be the $\ell_2$ minimizer of the error over the inliers i.e 
$$\ell' \defeq \underset{\ell \in \R^d}{\argmin} \sumn w_i'(y_i - \iprod{\ell,X_i})^2$$
%
\Pnote{data set must have the clean data and the rest.  Notation is  little inconsistent above,  $\ell'$ must be minimizer on clean data alone} 
Let $\sigma^2$ be a constant upper bounding the $\ell_2$ error  
$$\underset{\ell \in \R^d}{\argmin}  \sumn w_i' (y_i - \iprod{\ell',X_i})^2 \leq \sigma^2$$
Likewise, let $g$ be a constant such that the $\ell_4$ error of $\ell'$ is  
$$\underset{\ell \in \R^d}{\argmin} \sumn w_i'(y_i - \iprod{\ell',X_i})^4 \leq g\sigma^4$$
In the special case of Gaussian noise $\cN(0,\sigma^2)$ we have $g = 3$.  Then for any $d \in \mathbb{Z}^+$ sufficiently large, our algorithm recovers a list of estimates $L = \{\ell_1,...,\ell_A\}$ for $|L| = O\big((\frac{\rho}{\sigma})^{\log(\frac{1}{\beta})}\big)$ such that for some $\ell_i \in L$ we have

$$\norm{\ell_i - \ell'}_2 \leq O\left(\frac{\sigma}{\beta^{3/2}}\right)$$
with high probability over the data. 
If we regard $\frac{\rho}{\sigma}$ as a fixed constant then the list is of length $\poly(\frac{1}{\beta})$.   
Furthermore, our algorithm is \textit{efficient}, running in polynomial time $\poly(d,N)$ where we take $N = d^{O(\frac{1}{\beta^4})}$.  Here we take $N$ to be large enough to certify arbitrary closeness of the $K$'th empirical moments to the distributional moments of the covariates in $\ell_2$ norm for $K = O(\frac{1}{\beta^4})$.  That is to say, for any constant $\epsilon > 0$, and for $X_1,...,X_N \sim \cN(0,I_d)$ we have with high probability

$$
\Norm{\frac{1}{N}\sum_{i=1}^N X_i ^{\otimes \frac{K}{2}}(X_i^{\otimes \frac{K}{2}})^T - M_K}_F^2 \leq \epsilon
$$
where $M_K$ is the empirical $K$'th moment tensor of the spherical Gaussian.  For our analyses we take $d > \rho$ and $\epsilon = O(\sigma d^{-K})$.  For these settings of $N$ and $d$, and fixing $\rho,\sigma, \beta$ to be constants, we often write $o_d(1)$ without ambiguity.          


\Pnote{does exponent depend on $\beta$?}

Our approach is to run an SoS SDP, and then \textit{round} out the list.  We begin by describing the Robust Regression SoS SDP.  
\newpage
\begin{algorithm}[H] \label{algo:robustregressionSDP}
\SetAlgoLined
\KwResult{A degree $D$ pseudoexpectation functional $\pE_\zeta$}
 \textbf{Inputs}: $(\cD = \{X_i,y_i\}_{i=1}^N,\rho)$ data set, and upper bound on $\norm{\ell'}$\\
 \Pnote{directly list $\{(X_i,y_i)\}$ as inputs here.  It will be good to make a table like this, as self-contained as possible}
 \begin{eqnarray}
\begin{aligned}
& \underset{\text{degree D pseudoexpectations} \pE}{\text{minimize}}
& & \sum_{i=1}^N \pE[w_i]^2 \\
& \underset{\text{satisfies the polynomial system}}{\text{such that $\pE$}}
&  & (w_i^2 - w_i) = 0, \; i \in [N], \\
& & & \sum_{i=1}^N w_i - M  = 0, \; i \in [N], \\
%& & & \Norm{\frac{1}{M}\sum_{i=1}^N w_i X_i ^{\otimes \frac{t}{2}}(X_i^{\otimes \frac{t}{2}})^T - M_t}_F^2 - \epsilon \leq 0  , \;  t \in [K]\\
& & & \frac{1}{M}\sum_{i=1}^N w_i (\langle \ell,X_i\rangle - y_i)^4 - g\sigma^4) \leq 0, \\
& & & \frac{1}{M}\sum_{i=1}^N w_i (\langle \ell,X_i\rangle - y_i)^2 - \sigma^2\leq 0, \\
& & & \Norm{\frac{1}{M}\sum_{i=1}^N w_i (y_i - \iprod{\ell,X_i})X_i}_2^2 = 0, \\
& & & \norm{\ell}^2 - \rho^2 \leq 0\\
\end{aligned}
\end{eqnarray}\\
 \textbf{return}: $\pE_\zeta$
 \caption{RobustRegressionSDP}
\end{algorithm}

\Pnote{do we have to decide on a value of $\epsilon_t$ when we state the theorems?  if so, we can just make it explicit in the SDP.}

\Pnote{it seems like we use $D_4$ to denote $g$ later}

\Pnote{$\hat{\mu}$ in the above SDP is zero, correct?}
Let $\cP$ be the set of polynomial constraints of Robust Regression SDP.  We elaborate on the meaning of each constraint below, and we will often refer to them in our analyses according to the numbering below. 

\begin{enumerate}
    \item The first constraint $\{w_i^2 = w_i\}$ enforces $w_i \in \{0,1\}$ and we refer to it as the \textit{booleaness} constraint.
    \item The next constraint $\{\sum_{i=1}^N w_i - M\}$ ensures we select a $\beta$ fraction of the data set.
    \item The third constraint ensures that the pseudodistribution is over subsets with moments that match the distribution of the covariates. We refer to them as the \textit{moment} constraints.  
    \item The next constraints ensures the error incurred by $\ell$ is small, and we refer to them as the $\ell_2$ \textit{noise} constraint.
    \item Similarly, we have a $\ell_4$ \textit{noise} constraint.  
    \item We have the $\ell_2$ \textit{minimization} constraint, which sets $\ell$ equal to the $\ell_2$ minimizer of the selected $w_i$. \Pnote{$\ell_2$ minimizer of clean data?}
    \item Finally, the \textit{scaling} constraint restricts the length of $\ell$,  $\norm{\ell} \leq \rho^2$.  
\end{enumerate}
The RobustRegression SDP minimizes a convex objective which we refer to as \textit{Frobenius Minimization}.  This technique first used in the work of Hopkins and Steurer \cite{hopkins2017efficient}, ensures that the SDP solution is a convex combination over every possible solution to the system.
%
This turns out to be crucial.  To see why, consider an actual solution $W_\text{fake}$ consisting of variables $w_1,...,w_N \in \{0,1\}$ and $\ell \in \R^d$ satisfying $\cP$.  The distribution that places mass $1$ on $W_\text{fake}$ and no mass on the clean data is a valid distribution over the solutions to $\cP$ and therefore also a valid pseudodistribution.  Since we only have assumptions on less than half the data, a malicious $W_{fake}$ can be planted anywhere confounding our efforts to recover $\ell'$.  What we need is a way to produce a distribution over solutions to $\cP$ that is a convex combination over all the possible solutions.  The objective function $\sum_{i=1}^N \pE[w_i]^2$ is a strictly convex function, minimizing which ensures that SDP solution is spread over all solutions to $\cP$.  More precisely, we have the following guarantee.

\begin{lemma}\torestate{ \label{lem:FrobeniusMinimization}
(Frobenius minimization$\implies$Correlation)
Let $\cP$ be a polynomial system in variables $\{w_i\}_{i \in [N]}$ and a set of indeterminates $\{\ell_i \}_{i \in \N}$, that contains the set of inequalities:
\begin{align*}
w_i^2 = w_i & \forall i \in [N] & & 
\sum_i w_i = \beta N
\end{align*}
%
Let $\pE_\zeta: \R[\{w_i\}_{i \in [N]}, \{\ell\}]^{\leq D} \to \R$ denote a degree $D$ pseudoexpectation that satisfies $\cP$ and minimizes the norm $\norm{\pE_\zeta[ w]}$.
%
If $w'_i \in \{0,1\}$ and $\ell'$ is a satisfying assignment to $\cP$ then there is correlation with the inliers, 
\begin{equation}
\pE_\zeta\left[\frac{1}{M} \sum\limits_{i=1}^N w_iw_i' \right] \geq \beta     
\end{equation}}
\end{lemma}
We defer the proof of this statement to \prettyref{sec:Frobenius}\\
\textbf{Remark}: The lemma does not guarantee that $\pE_\zeta[(\iprod{w,w'} - \beta M)p(w,\ell)] \geq 0$ for all SoS polynomials $p(w,\ell)$ of deg($p(w,\ell)$) $\leq D-1$  .  That is to say, the guarantees of \pref{lem:FrobeniusMinimization} are only in pseudoexpectation.      

At this point we have found a pseudodistribution $\zeta$ satisfying $\cP$ that in pseudoexpectation is correlated with the inliers.  Pursuing a line of wishful thinking, we would like to sample from this pseudodistribution armed with access to its degree $D$ moments.  This is the algorithmic task of rounding the SDP solution, and it is chief intellectual thrust of this work.      

%
\Pnote{the description below doesn't provide much intuition.  It will be good to use the term: variance.  talk of pseudovariance (probably even define it here), and then use it to state the lemma as follows:
....
For the sake of exposition, let us say that $\pE$ corresponds an actual distribution over solutions to the polynomial system.  
%
Recall that the goal of the rounding algorithm is to recover the linear function $\ell$.
%
Suppose the variance of $\ell$ as a random variable is sufficiently small, then its expectation $\pE[\ell]$ is a good approximation to an actual solution.  
.....
}
For the sake of exposition, let us say that $\pE$ corresponds an actual distribution over solutions to the polynomial system.
Recall that the goal of the rounding algorithm is to recover the linear function $\ell'$.
Suppose the variance of $\ell'$ as a random variable is sufficiently small, then its expectation $\pE[\ell]$ is a good approximation to an actual solution.  Formally,


\begin{lemma}
\torestate{\label{lem:regressionSnapping}
Let $\eta \in [0,\frac{1}{2}]$ be a small constant.  
Let $\pE_\zeta$ be a degree $O(\frac{1}{\eta^4})$ pseudoexpectation satisfying the constraints of RobustRegressionSDP($\cD,\rho$).   Then if the pseudovariance of the estimator $\pE_\zeta[\ell]$ is small in every direction
\begin{align}\label{vr}
\max_u \pVar_\zeta[\iprod{\ell,u}] \leq \eta\rho^2 
\end{align}
and there is correlation with the inliers 
\begin{align}\label{fm}
\pE_\zeta\left[ \frac{1}{M}\sum_i w_i w'_i\right] \geq \beta
\end{align}
then our estimator satisfies,
\begin{align}
\norm{\pE[\ell] - \ell'} \leq \sqrt{ \frac{\eta\rho^2 + O(\frac{\sigma^2}{\eta^2})}{\beta}}
\end{align}
In particular, for $\eta = \frac{\beta}{8}$ and $\rho^2 > \Omega(\frac{\sigma^2}{\beta^3})$  the degree $O(\frac{1}{\beta^4})$ pseudoexpectation satisfies 
}
$$
\norm{\pE_\zeta[\ell] - \ell'} \leq \frac{\rho}{2}     
$$
\end{lemma}
\Pnote{using "slash left bracket"  and "slash right bracket", will ensure that the brackets are scaled to the required size, like in second equation above}

\Pnote{degree $1/\eta^4$ seems different from $1/\beta^5$ above?}

Provided we can take the pseudovariance down in every direction, the error guarantee 'contracts' from the trivial $\rho$ to $\frac{\rho}{2}$. It is then possible to iterate such a contraction procedure to achieve optimal error guarantees which is the subject of \pref{sec:iteration}.  
Without going into details, the proof of \pref{lem:regressionSnapping} critically relies on both the concentration and anticoncentration of the covariates.  For instance, if the covariates were drawn from a degenerate point distribution at the origin, then nothing can be inferred about $\ell'$.  In this sense, concentration is insufficient to recover $\ell'$ meaningfully.  To overcome this hurdle, we formalize what it means for a distribution to be SoS certifiably anticoncentrated. 

\textbf{Certifiable Anticoncentration}
As will become clear in \pref{sec:anticoncentration}, the smaller $\eta$ is, the harder it is for SoS to certify the bounds in the above lemma.  For purposes of anticoncentration, $\eta$ is a parameter representing an interval about the origin.  For any distribution $\cD$, we think of $\cD$ as being anticoncentrated if the mass of $\cD$ falling within the $\eta$ interval is small.  For example, in the case of $\cD = \cN(0,1)$, the mass within the $\eta$ interval is upper bounded by $\frac{\eta}{\sqrt{2\pi}}$.  Characterizing this "anticoncentration" of $\cD$ about the origin becomes increasingly difficult (higher degree) as $\eta$ falls, intuitively, because it requires a finer grained picture of the distribution $\cD$.  It turns out the $\cN(0,I_d)$ is $O(\frac{1}{\eta^4})$ SoS certifiably anticoncentrated the proof of which is detailed in \pref{sec:anticoncentration-distributions}.  That this proof is independent of the dimension $d$, along with the rounding algorithm, is what enables the list decoding to run in polynomial time.        
\\
\\
\Pnote{ the above description of anticoncentration seems out of place?  must be moved to a different place, where it is motivated.}


Now we move on to the actual statement of \pref{lem:regressionSnapping}.  In general, the variance of the SDP solution will not be small.  Thus, we will iteratively reduce the variance by conditioning on the $w_i$ variables.  Intuitively, we are conditioning on specific data points $(X_i,y_i)$ being part of the inliers ($w_i = 1$) or being part of the outliers ($w_i = 0$).  

\begin{comment}
the lemma states that if the pseudovariance of $\ell$ is small and there is correlation with the plant, then we have made progress towards $\ell'$.  By frobenius minimization, we already have correlation with the plant.  What remains is to find a pseudoexpectation for which $ \max_u \pVar_\zeta[\iprod{\ell,u}]$ is small.  We achieve this by iteratively \textit{conditioning} the SDP.
\end{comment}  
\Pnote{Reader doesn't know what the term "plant" refers to here, and "correlation with the plant".
%
Only thing the reader knows at this point is what we told him right before lemma 3.2,  "if variance is small then rounding is easy"  and Lemma 3.2 is some quantitative version of that.  We need to take the reader from there, something like:
"The variance of the SDP solution will not be small in general.  We will iteratively reduce the variance by conditioning on the $w_i$ variables.  Intuitively, we are conditioning on specific data points $X_i,y_i$ being part of the clean data"
-- again here "clean data" is a term we should only use if we stated it formally earlier.
}


Towards these ends, let $\pE_{1}, \pE_{2},..., \pE_{R}$ be a sequence of pseudoexpectations where $\pE_1$ is the output of RobustRegressionSDP($\cD,\rho$).  We want to define an algorithm to update $\pE_{t}$ to $\pE_{t+1}$ where $\max_u \pVar_{t+1}[\iprod{\ell,u}] < \max_u \pVar_{t}[\iprod{\ell,u}]$ so that eventually $\pE_{R} < \eta\rho^2$.   

let $\cQ_t$ be the pseudocovariance matrix defined 

$$\cQ_t = \pE_{t}[(\ell - \pE_t[\ell])(\ell - \pE_{t}[\ell])^T]$$
We have $\norm{\cQ_t}_{op} = \max_u \pVar_t[\iprod{\ell,u}]$.  Let's say we have a strategy $\cS$ for selecting a $w_j \in {w_1,...,w_N}$, and then apply the following update 
$$
\pE_{t+1} = \left\{
        \begin{array}{ll}
            \pE_{t}|_{w_j = 1} & \text{with probability} \pE_{t}[w_j]\\
            \pE_{t}|_{w_j = 0} &  \text{with probability} \pE_{t}[1 - w_j]\\
    \end{array}
\right.
$$
Let $b_j$ be a $\{0,1\}$ random variable satisfying $\Pr[b_j = 1] = \pE_t[w_j]$. 
We wish to argue that there is a large expected decrease in the direction of largest variance.   
\begin{align*}
        \norm{\cQ_t}_\text{op}  - \E_{\cS}\E_{b_j}\norm{\cQ_t\big|_{w_j = b_j}}_\text{op} > \text{large}
\end{align*}

\Pnote{good to remind reader what $_{\text{nuc}}$ norm means.  Also, the more standard notation is to use $\norm{Q}_{\infty}$ or $\norm{Q}$ for operator norm, $\norm{Q}_1$ for nuclear norm.}

Unfortunately, controlling $\norm{\cQ}_\text{op}$ is difficult.  We will instead control  
$\norm{\cQ}_\text{nuc}$, i.e trace norm, and prove 

\begin{align*}
        \norm{\cQ}_\text{nuc}  - \E_{\cS}\E_{b_j}\norm{\cQ\big|_{w_j = b_j}}_\text{nuc} \geq
        \Omega(\beta^3\rho^2)
\end{align*}
For the strategy $\cS$ defined below

\begin{lemma} (Variance Decrease Strategy) \torestate{\label{lem:regstrategy}
    Let $\pE_\zeta$ satisfy the pseudoexpectation constraints of RobustRegressionSDP($\cD,\rho$). Let $\cQ$ be the associated pseudocovariance matrix. Let $v$ be any direction in the unit ball $S^{d-1}$.  
    Let $\cS_v$ be a probability distribution over $[N]$\;
  where for any $j \in N$ we have 
  \begin{align*}
      \cS_v(j) \defeq \frac{\pVar_\zeta[w_j(y_j - \pE_\zeta[\langle \ell,X_i \rangle])\langle X_j,v\rangle]}{\sum_{i=1}^N \pVar_\zeta[w_j(y_j - \pE_\zeta[\langle \ell,X_i \rangle])\langle X_j,v\rangle]}
  \end{align*}
  
  Then for $M_4$ being the fourth moment matrix of the Gaussian defined in RobustRegressionSDP,  and for $\norm{\cQ}_{nuc} > \sigma^2\sqrt{g}$ we have   
  
  \begin{align*}
    \pVar_\zeta[\iprod{\ell,v}] -  \E_{j \sim S_v}\E_{b_j} \pVar_\zeta[\iprod{\ell,v}|w_j = b_j]
    \geq  \Omega\Big(\frac{\beta\pVar_\zeta[\iprod{\ell,v}]^2}{\norm{\cQ}_{nuc}}\Big)
\end{align*}
}    
\end{lemma}
\Pnote{Can $\cQ$ be any pseudocovariance matrix above?  or is it the pseudocovariance matrix of $\ell$?  Can we use the notation $\pVar[\ell]$ or something similar to denote pseudocovariance of $\ell$}
\Pnote{$M_4, \epsilon_4$ undefined above.  Also, ``largest eigenpair" does not seem like standard usage}

\Pnote{Does $v$ have to be the largest eigenvector for the above lemma?  If $v$ can be any eigenvector, we should just state for any.   Then, we can explain in text that the lemma lets one decrease the variance along a single direction, thereby decreasing the nuclear norm as follows, and state the corollary}
The above lemma allows the rounding algorithm to decrease the variance along a single direction, thereby decreasing the nuclear norm as follows.  
\begin{corollary}\label{cor:nnr} (Connecting variance decrease strategy to nuclear norm rounding)
For $(\lambda,v)$ being the largest eigenvalue/vector pair of $\cQ$, and $\cS_v$ defined in \pref{lem:regstrategy}. Let $\gamma > 0$ be a constant. If  $\norm{\cQ}_\text{op} \geq \gamma$ and $\norm{\cQ}_{nuc} > \sigma^2\sqrt{g}$, then
\begin{align*}
        \norm{\cQ}_\text{nuc}  - \E_{j \sim S_v}\E_{b_j}\norm{\cQ\big|_{w_j = b_j}}_\text{nuc} \geq \Omega\left(\frac{\beta\gamma^2}{\rho^2}\right)
    \end{align*}  
In particular, for $\gamma = \eta\rho^2$, we have  
 
 \begin{align*}
        \norm{\cQ}_\text{nuc}  - \E_{j \sim \cS_v}\E_{b_j}\norm{\cQ\big|_{w_j = b_j}}_\text{nuc} \geq
        \Omega(\beta\eta^2\rho^2)
    \end{align*}

 
\end{corollary}
The corollary establishes a win-win.  Either $\norm{\cQ}_{op} < \gamma$ in which case the variance of our estimator is small in every direction, or we can round and decrease an upper bound on $\norm{\cQ}_{op}$.  We defer the proof of \pref{lem:regstrategy} to \pref{sec:reg-rounding} and the proof of \pref{cor:nnr} to section \pref{sec:conditioning}.  

\Pnote{what is the following intuition for?  it appears to be for the entire algorithm and not the above corollary/lemma.  We should have it at a place where we describe the overall strategy, or tell the reader that we are describing the intuition behind the overall algorithm}

Taken together, the conditioning strategy iteratively chases the variance down by selecting the direction of largest variance in the pseudocovariance of our estimator, and conditions on the $w_j$ exhibiting the largest scaled variance.        

We are now ready to state our main algorithm and prove the main result of this section 

\Pnote{what is $\ell'$ in the theorem statement below? we should say, for any integral solution $\ell'$, we recover something close to $\ell'$ with probability $\beta/160$}
\begin{algorithm}[H] \label{algo:regressionroundtree}
\SetAlgoLined
\KwResult{a $d$ dimensional hyperplane}
 \textbf{Inputs}: $(\pE_1,\rho)$ The output of RobustRegressionSDP and the scaling parameter\\
 \For{$t = 1:O(\frac{1}{\eta^2\beta^2})$}{
  Let $\cQ_t = \pE_t[(\ell - \pE_t[\ell])(\ell - \pE_t[\ell])^T]$ be the pseudocovariance matrix of the estimator $\ell$\\
 \text{Let }$(\lambda,v)$\text{ be top eigenvalue/vector of }$\cQ_t$ \\
 \eIf{ $\lambda > \eta\rho^2$}{
  Let $\cS_v$ be a probability distribution over $[N]$\;
  Where for any $j \in N$ we have $\cS_v(j) \defeq \frac{\pVar_t[w_j(y_j - \pE_t[\langle \ell,X_i \rangle])\langle X_j,v\rangle]}{\sum_{i=1}^N \pVar_t[w_j(y_j - \pE_h[\langle \ell,X_i \rangle])\langle X_j,v\rangle]}$ \\
  Sample $j \sim \cS_v$ \\
  Sample $b_j \in $ Bern($\pE_t[w_j]$)\\
  Let $\pE_{t+1} = \pE_t\big|_{w_j = b_j}$\\
 }
 {
 \textbf{return:} $\pE_t[\ell]$
 }
 }
 \caption{Regression Rounding Algorithm}
\end{algorithm}


\begin{theorem} \label{thm:main-regression-estimation}
    Let $\ell'$ be a solution to the constraints of RobustRegressionSDP.  Let $\eta$ be a constant greater than $0$.  Let $\pE_{\zeta}$ be the output of $\text{RobustRegressionSDP}(\cD,\rho)$ for degree $D = O\Big(\max(\frac{1}{\beta^2\eta^2},\frac{1}{\eta^4})\Big) $.  Then after $R = O(\frac{1}{\beta^2\eta^2})$ rounds of updates according to the strategy $\cS$ in \pref{lem:regstrategy}, the resulting pseudoexpectation, which we denote $\pE_R$, satisfies
    $$ \norm{\pE_{R}[\ell] - \ell'} \leq \sqrt{\frac{\eta\rho^2 + O\big(\frac{\sigma^2}{\eta^2})}{\beta}}$$
    with probability greater than $\Omega(\beta)$ over the randomness in the algorithm.  In particular for $\eta = \Omega(\beta)$ and for $\rho^2 \geq \Omega\big(\frac{\sigma^2}{\beta^3} \big)$, the degree $D = O(\frac{1}{\beta^4})$ pseudoexpectation satisfies  
    $$ \norm{\pE_{R}[\ell] - \ell'} \leq \frac{\rho}{2}$$
\end{theorem}

\textbf{Remark}:    
\Pnote{technically, this is a list decoding algorithm already, since one gets the full list by running the algorithm many many times, and boosting the probability that something close to $\ell'$ appears.  Alternately, one can think of going over all possibilities for the random choices made by the algorithm}

As stated, \pref{thm:main-regression-estimation} takes down the error guarantee to $\frac{\rho}{2}$ and is not yet an iterative algorithm that obtains the optimal error guarantees, yet it contains most of the elements of the full algorithm.  Issues concerning iteration are the subject of the next section on algorithms.          

\begin{proof}
We now have all the tools to prove \pref{thm:main-regression-estimation}.  By frobenius minimization \pref{lem:FrobeniusMinimization} we have, 
$$\pE_{\zeta}[\sumn w_iw_i'] \geq \beta$$ 
Now we show that after $R$ rounds of conditioning,
$$ \max_{u \in \cS^{d-1}} \pVar_{\zeta,R}[\iprod{\ell,u}] \leq  \eta\rho^2$$

To apply \pref{lem:regressionSnapping} we iteratively round according to $\cS_v$ in  \pref{lem:regstrategy} to decrease $\norm{\cQ}_{nuc}$.  For $\norm{\cQ}_{op} > \eta\rho^2$, \pref{cor:nnr} gives us 

\begin{align*}
        \norm{\cQ}_\text{nuc}  - \E_{j \sim S_v}\E_{b_j}\norm{\cQ\big|_{w_j = b_j}}_\text{nuc} \geq \Omega(\beta\eta^2\rho^2)
\end{align*}  

\Pnote{too many sentences starting with words like Or, Either, Where,  perhaps we should reduce that a bit}

We aim to show that after $R = O(\frac{1}{\beta^2\eta^2})$ iterations, the algorithm outputs $\norm{\cQ_R}_\text{nuc} \leq \eta\rho^2$ with probability greater than $1 - \frac{\beta}{4}$ over the randomness in the selection strategy and ${0,1}$ conditionings.  We denote the probability and expectation over the randomness in the algorithm $\Pr_\cA[\cdot]$ and $\E_\cA[\cdot]$ respectively.  Thus, to prove the following  
$$\Pr_{\cA}[\norm{\cQ_R}_{op} \leq \eta\rho^2] \geq 1 - \frac{\beta}{4}$$
we proceed by contradiction.  Suppose that at each iteration of $t = 1,2,...,R$, that $\norm{\cQ_t}_\text{op} > \eta\rho^2$ with probability greater than $\frac{\beta}{4}$.  Then in expectation over $\cS$ we have that each round of conditioning decreases $\norm{\cQ}_\text{nuc}$ by $\frac{\beta}{4}$ (the probability that the assumption in \ref{eq:overview1} holds) times $\Omega(\beta\eta^2\rho^2)$ (the expected decrease in \ref{eq:overview1}).  Thus, 

\begin{align}\label{eq:overview1}
\E_{\cA}[\norm{\cQ_t}_\text{nuc}] - \E_{\cA}[\norm{\cQ_{t+1}}_\text{nuc}] \geq \Pr_{\cA}[\norm{\cQ_t}_\text{op} \geq \eta\rho^2]\cdot \Omega(\beta\eta^2\rho^2) \geq \Omega(\beta^2\eta^2\rho^2)
\end{align}

We also know that the initial pseudocovariance is upper bounded in nuclear norm i.e  

\begin{align}\label{eq:overview2}
\norm{\cQ_{\zeta}}_\text{nuc} = \pE_\zeta[\norm{\ell - \pE_\zeta[\ell]}^2] = \pE_\zeta[\norm{\ell}^2] - \pE_\zeta[\norm{\ell}]^2 \leq \pE_\zeta[\norm{\ell}^2] \leq \rho^2
\end{align}

Where the last inequality is an application of the scaling constraint (7).  Thus, putting together \ref{eq:overview1} and \ref{eq:overview2} after $R = O(\frac{\rho^2}{\beta^2\eta^2\rho^2}) = O(\frac{1}{\beta^2\eta^2})$ iterations,   $\E_{\cA}[\norm{\cQ_R}_\text{nuc}] \leq 0$ which is impossible because $\norm{\cQ_R}_\text{nuc} = \pE_R[\norm{\ell - \pE_R[\ell]}^2] \geq 0$.  Thus our assumption is false, and   $\Pr_{\cA}[\norm{\cQ_R}_{op} \leq \eta\rho^2] \geq 1 - \frac{\beta}{4}$ as desired.
\begin{comment}
Then after 
$$R =  O\Big(\frac{\rho^2 - \frac{\beta\eta\rho^2}{4}}{\beta^3\eta^2\rho^2}\Big) = O\Big(\frac{1}{\beta^3\eta^2}\Big)$$ iterations we have that in expectation, one of the following two possibilities occur.  Either, at some iteration $\norm{\cQ}_{op} \leq \frac{\beta\eta\rho^2}{4}$ in which case we have successfully decreased the variance.  Or, we made progress in expectation at each iteration so that   

$$\norm{\cQ_{\zeta,R}}_\text{nuc} \leq \frac{\beta\eta\rho^2}{4}$$
Using the fact that operator norm is upper bounded by nuclear norm we obtain 
$$\norm{\cQ_{\zeta,R}}_\text{op} \leq \frac{\beta\eta\rho^2}{4}$$
Either way, we have successfully brought down the variance in expectation over the randomness in the strategy and the selection of $\{0,1\}$ conditionings.  Thus by Markov's we have that \Pnote{markovs with capital M?}
$$\Pr_{\cA}[\norm{\cQ_R}_{op} \geq \eta\rho^2] \leq \frac{\beta}{4}$$
So $\Pr_{\cA}[\norm{\cQ_R}_{op} \leq \eta\rho^2] \geq 1 - \frac{\beta}{4}$.

\Pnote{in the above Markov, what is the probability over?  is the previous inequality missing an $\E$ over something}
\end{comment}

We also know by the law of total pseudoexpectation that in expectation over the selection strategy and ${0,1}$ conditionings,    
\[ \E_{\cA}\left[\pE_{R}\left[\sumn w_iw_i'\right]\right]= \pE_{\zeta}\left[\sumn w_iw_i'\right] \geq \beta \]
\Pnote{ $slash left bracket$  and $slash right bracket$} Note that this is a generic fact that is true regardless of which conditioning strategy we choose.  Thus by Markov for random variables taking values in $[0,1]$ we have 

$$\Pr_{\cA}\left[\pE_{R}\left[\sumn w_iw_i'\right] \geq \frac{\beta}{2}\right] \geq \frac{\beta}{2}$$
Now that we know $\Pr_{\cA}[\norm{\cQ_R}_{op} \leq \eta\rho^2] \geq 1 - \frac{\beta}{4}$ and $\Pr_{\cA}\left[\pE_{R}\left[\sumn w_iw_i'\right] \geq \frac{\beta}{2}\right] \geq \frac{\beta}{2}$, we conclude via union bound that the failure probability of both events is upper bounded by $\frac{\beta}{4} + 1 - \frac{\beta}{2} = 1 - \frac{\beta}{4}$.  Thus  
the conditions of \pref{lem:regressionSnapping} are satisfied with probability greater than $\frac{\beta}{4}$ in which case 
$$ \norm{\pE_{R}[\ell] - \ell'} \leq \sqrt{\frac{\eta\rho^2 + O\big(\frac{\sigma^2}{\eta^2})}{\beta}}$$
     In particular for $\eta = \Omega(\beta)$ and for $\rho^2 \geq \Omega\big(\frac{\sigma^2}{\beta^3} \big)$ we have  
     $$ \norm{\pE_{R}[\ell] - \ell'} \leq \frac{\rho}{2}$$

\Pnote{we should conclude, just to remind the reader why this is desired?}
\end{proof}
\begin{lemma}\torestate{\label{lem:roundtree}
Running Algorithm \pref{algo:regressionroundtree} a total of $O(\frac{1}{\beta})$ times produces a list $L = \{\ell_1,...,\ell_{O(\frac{1}{\beta})}\}$ such that with probability 1 - c, there exists a list element $\ell_i \in L$ satisfying 
$\norm{\ell_i - \ell'} \leq \frac{\rho}{2}$
where $c$ is a small constant. Minor modifications enable the algorithm to succeed with high probability. } 
\end{lemma}
We defer the modifications required to succeed with high probability to the appendix. We proceed under the assumption that \pref{algo:regressionroundtree} outputs a list $L$ satisfying the guarantees in \pref{lem:roundtree} with high probability. For variety, we present the mean estimation algorithms with these modifications in place.   
\Pnote{ $\eta$ needs to be quantified in above lemma?}







==> sosListDecoding.tex <==
\section{Frobenius Minimization}

\begin{comment}

\begin{theorem}\label{center}

For any pseudodistribution $\zeta$ output by RobustMeanSDP the following inequality holds 
\begin{equation}
\norm{\pE_\zeta[\hu] - \mu}_2 \leq \sqrt{\frac{2\max_{u \in \cS^{d-1}}\pE_\zeta[\langle \pE_\zeta[\hu] - \hu,u\rangle^2] + \pE_\zeta[\sumn w_iw_i'||\hu - \mu||^2]}{\pE_\zeta[\sumn w_iw_i']}}
\end{equation}

Similarly, for any pseudodistribution $\zeta$ output by RobustRegressionSDP the following inequality holds  
\begin{equation}
\norm{\pE_\zeta[\ell] - \ell'}_2 \leq \sqrt{\frac{2\max_{u \in \cS^{d-1}}\pE_\zeta[\langle \pE_\zeta[\ell] - \ell,u\rangle^2] + \pE_\zeta[\sumn w_iw_i'||\ell - \ell'||^2]}{\pE_\zeta[\sumn w_iw_i']}}
\end{equation}

\end{theorem}
\begin{proof}
The proof of \ref{center} goes the same for both mean estimation and regression.  For mean estimation let $R := \hu$ and for regression let $R := \ell$. We have, 
\begin{align*}
    \pE[\sumn w_iw_i']\langle \pE[R] - R',u\rangle^2 = \pE[\sumn w_iw_i'\langle \pE[R] - R',u\rangle^2]
\end{align*}
Applying triangle inequality 
\begin{align*}
    =\pE[\sumn w_iw_i'\langle \pE[R] - R + R - R',u\rangle^2] \leq 2
    \pE[\sumn w_iw_i'\langle \pE[R] - R,u\rangle^2]  + 2\pE[\sumn w_iw_i'\langle R - R',u\rangle^2]
\end{align*}

Summing over $w_iw_i'$ in the first term to obtain global correlation, we have

\begin{align*}
    \leq 2
    \pE[\langle \pE[R] - R,u\rangle^2]  + 2\pE[\sumn w_iw_i'\langle R - R',u\rangle^2]
\end{align*}

by Cauchy-Schwarz on the second term we obtain 

\begin{align*}
    \pE[\sumn w_iw_i']\langle \pE[R] - R',u\rangle^2 \leq 2
    \pE[\langle \pE[R] - R,u\rangle^2]  + 2\pE[\sumn w_iw_i'||R - R'||^2]
\end{align*}

rearranging the terms we obtain 

\begin{align*}
    \langle \pE_\zeta[R] - R', u \rangle \leq \sqrt{\frac{\pE[\langle \pE[R] - R,u\rangle^2] + \pE_\zeta[\sumn w_iw_i'||R - R'||^2]}{\pE_\zeta[\sumn w_iw_i']}}
\end{align*}
Maximizing over all $u \in \cS^{d-1}$
\begin{align*}
    \norm{\pE_\zeta[R] - R'}_2 \leq \sqrt{\frac{\max_{u \in \cS^{d-1}}\pE[\langle \pE[R] - R,u\rangle^2] + \pE_\zeta[\sumn w_iw_i'||R - R'||^2]}{\pE_\zeta[\sumn w_iw_i']}}
\end{align*}

as desired
\end{proof}
\noindent
The above theorem reduces the problem of finding a pseudodistribution for which $\norm{\pE_\zeta[R] - R'}_2$ is small to that of upper bounding $\max_{u \in \cS^{d-1}}\pE_\zeta[\langle \pE_\zeta[R] - R,u\rangle^2]$ and $\pE_\zeta[\sumn w_iw_i'||R - R'||^2]$ and lower bounding $\pE_\zeta[\sumn w_iw_i']$.  Henceforth, we will loosely refer to 
$\max_{u \in \cS^{d-1}}\pE_\zeta[\langle \pE_\zeta[R] - R,u\rangle^2]$ as global correlation, and $\pE_\zeta[\sumn w_iw_i'||R - R'||^2]$ as the "bias" term.  Global correlation captures the variance of the estimator $R$.  If $R$ is concentrated, then global correlation is small and the estimator $R$ is close to its expectation $\pE_\zeta[R]$.  The "bias" term intuitively captures how far $\pE_\zeta[R]$ is from $R'$.   
\end{comment}

\subsection{Frobenius Norm Minimization} \label{sec:Frobenius}

    \restatelemma{lem:FrobeniusMinimization}


\begin{proof}
Let $\pE_P$ denote the pseudo-expectation operator corresponding to the actual assignment $\{w'_i\}_{i \in [N]}$ and $\{\ell'\}$.
%
Note that $\pE_P$ is an actual expectation over an assignment satisfying the polynomial constraints.
%
For a constant $\kappa \in [0,1]$, let us consider the pseudoexpectation operator $\pE_R$ defined as follows for a polynomial $p(w)$,
$$\pE_R  \defeq  \kappa \pE_P + (1-\kappa)\pE_D$$
%
Since $\pE_D$ is the pseudoexpecation operator that minimizes $\norm{\pE_D[w]}$, we get that
\begin{equation}\label{eqfm1}
\iprod{\pE_R[w], \pE_R[w]} \geq \iprod{\pE_D[w], \pE_D[w]}
%\sum\limits_{i=1}^N (\pe_R[w_i])^2 \geq  \sum\limits_{i=1}^N (\pe_D[w_i])^2 
\end{equation}

Expanding the LHS with the definition of $R$ we have
\begin{align*}
(1-\kappa)^2 \cdot \iprod{\pE_D[w], \pE_D[w]} + 2 \kappa (1-\kappa) \iprod{\pE_D[w], \pE_P[w]} + \kappa^2 \iprod{\pE_P[w],\pE_P[w]} \geq \iprod{\pE_D[w], \pE_D[w]}
\end{align*}
Rearranging the terms we get
\begin{align*}
  \iprod{\pE_D[w], \pE_P[w]}  \geq \frac{1}{2 \kappa(1-\kappa)} \left((2\kappa - \kappa^2)\iprod{\pE_D[w], \pE_D[w]} -\kappa^2 \iprod{\pE_P[w],\pE_P[w]}\right)
\end{align*}
By definition, we have that $\iprod{\pE_P[w], \pE_P[w]} = \sum_i w_i^{'2} = \beta N$.  By Cauchy-Schwartz inequality, $\iprod{\pE_D[w],\pE_D[w]} \geq \frac{1}{N} \left(\sum_i \pE_D[w_i]\right)^2 = \frac{1}{N} (\beta N)^2 = \beta^2 N $.  Substituting these bounds back we get that,
\begin{align*}
    \iprod{\pE_D[w], \pE_P[w]} \geq \frac{\left((2\kappa - \kappa^2)\beta^2 -\kappa^2 \beta\right)}{2 \kappa(1-\kappa)}  \cdot N 
\end{align*}
Taking limits as $\kappa \to 0$, we get the desired result.

\end{proof}

\iffalse
$$\sum\limits_{i=1}^N (\pE_R[w_i])^2
 = \sum\limits_{i=1}^N (\kappa \pE_P[w_i] + (1-\kappa)\pE_D[w_i])^2$$
 Expanding the square
$$ = (1 - \kappa)^2 \sum\limits_{i=1}^N (\pE_D[w_i])^2 + 2\kappa(1-\kappa)\sum\limits_{i=1}^N \pE_D[w_i]\pE_P[w_i] + \kappa^2\sum\limits_{i=1}^N \pE_P[w_i]^2$$
Using the definition of $\pE_P$
$$ =  (1 - \kappa)^2 \sum\limits_{i=1}^N (\pE_D[w_i])^2 + 2\kappa(1-\kappa)\sum\limits_{i=1}^N \pE_D[w_i]w'_i + \kappa^2 \sum_{i = 1}^N w'_i^2$$
$$=  (1 - \kappa)^2 \sum\limits_{i=1}^N (\pE_D[w_i])^2 + 2\kappa(1-\kappa)\pE_D[\sum\limits_{i=1}^N w_i w_i'] + \kappa^2 \beta N$$

Now we rewrite  \ref{eqfm1} as

\begin{equation}
    (1 - \kappa)^2 \sum\limits_{i=1}^N (\pE_D[w_i])^2 + 2\kappa(1-\kappa)\pE_D[\sum\limits_{i=1}^N w_i w_i'] + \kappa^2 \beta N \geq \sum\limits_{i=1}^N (\pE_D[w_i])^2
\end{equation}
Rearranging the terms we obtain
$$ 2\kappa(1-\kappa)\pE_D[\sum\limits_{i=1}^N w_i w_i'] + \kappa^2 \beta N \geq (2\kappa - \kappa^2)\sum\limits_{i=1}^N (\pE_D[w_i])^2$$
Dividing both sides by $\kappa$ (note $\kappa > 0$)
\begin{equation}\label{eqfm2}
    2(1-\kappa)\pE_D[\sum\limits_{i=1}^N w_i w_i'] + \kappa \beta N \geq (2 - \kappa)\sum\limits_{i=1}^N (\pE_D[w_i])^2
\end{equation}
\Pnote{it might be good to call this Cauchy-Schwartz instead of Jensen's}
Note that by Jensen's inequality and applying the constraint $\sum\limits_{i=1}^N w_i = \beta N$, the RHS is greater than
$$ (2 - \kappa)\sum\limits_{i=1}^N (\pE_D[w_i])^2 = (2 - \kappa)N\frac{1}{N}\sum\limits_{i=1}^N (\pE_D[w_i])^2 \geq
(2 - \kappa)N(\frac{1}{N} \sum\limits_{i=1}^N\pE_D[w_i])^2$$
$$ =  (2 - \kappa)N(\frac{1}{N}\pE_D[\sum\limits_{i=1}^N w_i])^2$$
$$ = (2 - \kappa)\beta^2N $$
Thus rewriting \ref{eqfm2} we obtain
$$2(1-\kappa)\pE_D[\sum\limits_{i=1}^N w_i w_i'] + \kappa \beta N \geq (2 - \kappa)\beta^2 N$$
which for sufficiently small, but positive values of $\kappa$ gives
$$\pE_D[\sum\limits_{i=1}^N w_i w_i'] \geq \beta^2 N $$
as desired.
\fi


%Pseudodistributions are relaxations of actual distributions.  Thus, let $P$ be the pseudodistribution that is an actual distribution with support over the plant and nothing else.  Let $w_p$ denote the set of indices in the planted solution.  Let $D$ denote the pseudodistribution outputted by List-Decoding SDP.  Let pseudodistribution $R$ be a convex combination of $P$ and $D$ i.e for some constant $\kappa \in [0,1]$ and any polynomial $p(w): \{0,1\}^N \rightarrow \R$, we have
%Note that the following analysis makes no mention of the data $\{X_i\}_{i \in [N]}$.
%
%By the frobenius minimization, we know the objective value of $R$ is greater than the objective value for $D$.
%\begin{equation}\label{eqfm1}
%\sum\limits_{i=1}^N (\pe_R[w_i])^2 \geq  \sum\limits_{i=1}^N (\pe_D[w_i])^2 
%\end{equation}

 
